A Modal-Space Formulation for Momentum Observer Contact Estimation and Effects of Uncertainty for Continuum Robots

Contact detection for continuum and soft robots has been limited in past works to statics or kinematics-based methods with assumed circular bending curvature or known bending profiles. In this paper, we adapt the generalized momentum observer contact estimation method to continuum robots. This is made possible by leveraging recent results for real-time shape sensing of continuum robots along with a modal-space representation of the robot dynamics. In addition to presenting an approach for estimating the generalized forces due to contact via a momentum observer, we present a constrained optimization method to identify the wrench imparted on the robot during contact. We also present an approach for investigating the effects of unmodeled deviations in the robot's dynamic state on the contact detection method and we validate our algorithm by simulations and experiments. We also compare the performance of the momentum observer to the joint force deviation method, a direct estimation approach using the robot's full dynamic model. We also demonstrate a basic extension of the method to multisegment continuum robots. Results presented in this work extend dynamic contact detection to the domain of continuum and soft robots and can be used to improve the safety of large-scale continuum robots for human-robot collaboration.

==> preamble/bios.tex <==
\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/png/Garrison_profile.jpg}}]
{Garrison L.H. Johnston}
received the B.S. degree in mechanical engineering from the Rensselaer Polytechnic Institute (RPI), Troy, NY, USA, in 2018. He is currently pursuing the Ph.D. degree in mechanical engineering with Vanderbilt University, Nashville, TN, USA. His current research interests include human–robot interaction, continuum robot modeling and control, and mechanism design.
\end{IEEEbiography}
\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/png/Neel_profile.jpg}}]
{Neel Shihora}
received the B.Tech. degree in mechanical engineering from the National Institute of Technology (NIT) Surat, Gujarat, India. He is currently pursuing the Ph.D. degree in mechanical engineering with Vanderbilt University, Nashville, TN, USA. His current research interests include surgical robot design and modeling, robot assistance for remote interventions, and haptics for surgical robotics.  
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/pdf/nabil_simaan_profile.pdf}}]
{Nabil Simaan}
(Fellow, IEEE) received the Ph.D. degree in mechanical engineering from the Technion–Israel Institute of Technology, Haifa, Israel, in 2002.
%
\par During 2003, he was a Postdoctoral Research Scientist with Johns Hopkins University National Science Foundation (NSF), Computer-Integrated Surgical Systems and Technology Engineering Research Center (ERC-CISST), Maryland, USA. In 2005, he joined Columbia University, New York, NY, USA. His research interests include medical robotics, kinematics, robot modeling and control and human–robot
interaction.
%
\par He was the recipient of the NSF Career award for young investigators to design new algorithms and robots for safe interaction with the anatomy in 2009. In Fall 2010 he joined Vanderbilt University, Nashville, TN, USA. In 2020, he was named an IEEE Fellow for contributions to dexterous continuum robotics. In 2021, he was elected Fellow of the ASME for contributions to continuum and soft robotics for surgery
\end{IEEEbiography}


==> tex_content/dynamics_review.tex <==
\subsection{Previous Works on Continuum Robot Dynamic Modeling}
\GJ{From my proposal, need to update}
Although we don't claim to make a contribution to dynamic modeling of continuum robots, dynamic modeling of continuum robots is a necessary step to implementing the GMO for continuum robots. For this purpose, we will present a brief literature review of dynamic models for continuum robots. This literature review will help select a model to be used for the proposed work. There have been many techniques used to generate dynamic models of continuum robots presented in the literature. Perhaps the most common is the Euler-Lagrange method \cite{Book1984_recursive_lagrangian,Tatlicioglu2007_extensible_continuum_dynamics,Tatlicioglu2007_planar_continuum_dynamics,Godage2011_shape_function_variable_length_dynamics,He2013_lagrange,Falkenhahn2014_cc_lagrange,Roy2016_dynamic_effect_collision}. In \cite{Chirikjian1994_hyperredundant_dynamics}, Chirikjian used continuum mechanics to derive the equations of motion of curvilinear snake robots. Other dynamic modeling techniques that have been used in the literature include the recursive Newton-Euler method \cite{Khalil2005_recursive_newton_euler,Kang2011_recursive_newton_euler}, Hamilton's principle \cite{Gravagne2003_large_deflection_continuum}, Kane's method \cite{Everett1989_kanes_method}, lumped parameter models \cite{Jung2011_lumped_parameter}, virtual power modeling \cite{Rone2014_virtual_power}, Cosserat rod theory \cite{Till2019_cosserat_dynamics}, pseudo-rigid body models \cite{Mochiyama2003_flexible_dynamics}, and  mass-spring-damper networks \cite{Guo2015_continuum_dynamics}.
